Toward Adaptive Causal Consistency for Replicated Data Stores

Causal consistency for key-value stores has two main requirements (1) do not make a version visible if some of its dependencies are invisible as it may violate causal consistency in the future and (2) make a version visible as soon as possible so that clients have the most recent information (to the extent feasible). These two requirements conflict with each other. Existing key-value stores that provide causal consistency (or detection of causal violation) utilize a static approach in the trade-off between these requirements. Depending upon the choice, it assists some applications and penalizes some applications. We propose an alternative where the system provides a set of tracking groups and checking groups. This allows the application to choose the settings that are most suitable for that application. Furthermore, these groups can be dynamically changed based on application requirements.

==> related.tex <==
\section{Related Work}

There are other configurable protocols that like \name, help us deal with trade-offs. Occult \cite{occult} is one of such protocols that lets us trade-off between having lower metadata overhead and lower update visibility latency. However, the trade-off needs to be done by the developers at time of starting the protocol. Thus, the protocol does not adapt itself to answer to the changes of the system. Occult also suffers from a strict data placement schema. It requires full replicas to have a full copy of the data, and clients also must access the master replicas to write new versions. We believe Occult also will benefit from adaptive approach. 

Quorum-based systems like DynamoDB \cite{dynamo} or Voldemore provide an approach to face the trade-off between availability and consistency. An interesting feature of these systems is that they let us to trade-off on the run-time, as each query can specify its own level of consistency. However, unlike our approach that relies on automatic adaptation by the servers, DynamoDB and Voldemort require clients to specify the level of consistency that they want. Quorum-based consistency would also benefit from automatic adaptation.  

There is another adaptive work (I need to read, 1998 paper). 


